Regression Transformer: Concurrent sequence regression and generation for molecular language modeling

Despite significant progress of generative models in the natural sciences, their controllability remains challenging. One fundamentally missing aspect of molecular or protein generative models is an inductive bias that can reflect continuous properties of interest. To that end, we propose the Regression Transformer (RT), a novel method that abstracts regression as a conditional sequence modeling problem. This introduces a new paradigm of multitask language models which seamlessly bridge sequence regression and conditional sequence generation. We thoroughly demonstrate that, despite using a nominal-scale training objective, the RT matches or surpasses the performance of conventional regression models in property prediction tasks of small molecules, proteins and chemical reactions. Critically, priming the same model with continuous properties yields a highly competitive conditional generative model that outperforms specialized approaches in a substructure-constrained, property-driven molecule generation benchmark. Our dichotomous approach is facilitated by a novel, alternating training scheme that enables the model to decorate seed sequences by desired properties, e.g., to optimize reaction yield. In sum, the RT is the first report of a multitask model that concurrently excels at predictive and generative tasks in biochemistry. This finds particular application in property-driven, local exploration of the chemical or protein space and could pave the road toward foundation models in material design. The code to reproduce all experiments of the paper is available at: https://github.com/IBM/regression-transformer

==> intro_old.tex <==
%\subsection{On the decline of inductive biases}
Transformers~\citep{vaswani2017attention} are now ubiquitous in natural language processing (NLP) and have also enjoyed large success in molecular~\citep{schwaller2019molecular,schwaller2021mapping,schwaller2021extraction}
%,wang2019smiles
and protein language modeling~\citep{rives2021biological,jumper2021highly}.
The invention of Transformers was in alignment with the steady decline of inductive biases in ML, a trend that started with the rise of deep learning:
% in 2012
%Since the breakthrough of deep learning in 2012~\citep{krizhevsky2012imagenet}, we have witnessed a steady trend toward lowering inductive biases in deep networks.
CNNs outperformed traditional feature descriptors in object recognition~\citep{krizhevsky2012imagenet}, self-attention generalized dense layers to learn sample-dependent instead of static affine transformations~\citep{luong2015effective} and Transformers exploited self-attention 
%to leave behind the \textit{recurrent inductive bias} of RNNs
to supersede RNNs as
%(sequentiality, memory bottleneck and recursion
%~\citep{abnar2020transferring})
%and became 
the de-facto standard in NLP.
%~\citep{reis2021transformers}.
The success of vision transformers has questioned the need for translation equivariance 
%and convolutions 
in image processing~\citep{ramachandran2019stand} and now, even frozen Transformers pretrained on text achieve SOTA results in object detection and protein classification~\citep{lu2021pretrained}.
%Ultimately, transformers are nowadays' most generic models: graph neural networks (GNN) with multihead attention as neighborhood aggregation function operating on fully connected graphs~\citep{joshi2020transformers}.
Given that Transformers are today's most generic model\footnote{graph neural networks with multihead attention as neighborhood aggregation on complete graphs
%~\citep{joshi2020transformers}
},
it is not surprising that attempts have been made to abstract entire domains like RL to sequence modeling in order to leverage Transformers~\citep{chen2021decision}.
%Apart from these architectural advances, techniques like masked language modeling~(MLM,~\cite{devlin2019bert}) and its successor permutation language modeling~(PLM,~\cite{yang2019xlnet}) have enabled large-scale unsupervised pretraining of transformers that led to significant improvements on downstream predictive and generative tasks. 
%Due to the success of transformers, abstracting existing problem formulations to sequence modeling is not entirely novel, e.g., the Decision Transformer~\citep{chen2021decision} casts reinforcement learning (RL) as conditional sequence modeling and thus allows to generate appropriate actions by conditioning on desired rewards.

%
\begin{figure*}[!htb]
\centering
\includegraphics[width=1\linewidth]{figures/overview_v5.pdf}
\caption{
\begin{small}
\textbf{Overview of Regression Transformer (RT).}
The RT is a multitask language model designed to handle combinations of text and numbers.
\textbf{a)} Traditional approach in generative chemistry: property predictors and generative models are trained independently from another.
\textbf{b)} Our approach:  Training the RT yields a dichotomous model that seamlessly switches between property prediction and conditional text generation.
%\textit{Blue stream (top):} If the positions between the property tag~\texttt{<QED>} and the delimiter~\texttt{|} are masked, the RT predicts a series of numerical tokens that can be converted to a float.
%\textit{Yellow stream (bottom):} Instead, if textual tokens are 
Dependent on the mask location, the same model either predicts numerical tokens given textual tokens, thus performing a regression task \textit{(blue stream, top)}; or predicts textual tokens given both numerical and textual tokens, thus performing a property-driven conditional generation \textit{(yellow stream, bottom)}.
\textbf{c)} - \textbf{f)}:
This novel formulation finds application across a wide range of domains. 
We demonstrate the flexibility of the RT in predictive and generative tasks in modeling small molecules, proteins, chemical reactions.
It can even be applied on NLP tasks such as modeling humour.
\end{small}
}
\label{fig:graphicalabstract}
\end{figure*}
%
%
% \vspace{-1mm}
% \paragraph{The Regression Transformer.}
% \vspace{-1mm}
A provocative next step toward reducing inductive biases might be to refrain from explicitly modeling target variables as functions of input variables.
Instead of following this discriminative modelling approach when tuning task-specific language heads in Transformers, learning the joint distribution over input and target variables could effectively further blur the lines between predictive and conditional generative models.
The feasibility of such approach can be assessed via permutation language modeling (PLM~\citep{yang2019xlnet}), an adaption of masked-language-modeling.
%Here, we thus investigate whether the benefits of such pretraining objectives extend to numerically labelled text datasets and facilitate the development of multitask models.
%
%Based on the above, a natural question is whether the benefits of MLM/PLM pretraining extend to numerically labelled text datasets, such as regression tasks.
%Based on the above, one natural question is whether the benefits of MLM/PLM pretraining extend to numerically labelled text datasets and regression tasks.
%

Here, we reformulate regression as a sequence modeling task of textual tokens. 
We propose the Regression Transformer (RT), a novel multitask model that can be trained on combinations of numerical and textual tokens (\autoref{fig:graphicalabstract}).
This circumvents the canonical way of addressing regression in Transformers, i.e., tuning a designated regression head~\citep{devlin2019bert}.
Despite solely relying on tokenization of numbers and cross-entropy loss, the RT can successfully solve regression tasks.
%(i.e., predict continuous properties of sequences).
Notably, the same model can conditionally generate text sequences given continuous properties.
This is achieved simply by moving the \texttt{[MASK]} location, does not require finetuning specific heads and thus constitutes a true multitask model.
To equip the RT with an inductive bias for handling floating-point properties, numbers are first tokenized into a sequence of tokens preserving the decimal order.
We then devise numerical encodings to inform the model about the semantic proximity of these tokens.
To allow for concurrent optimization of regression and conditional generation, we derive a PLM-inspired, alternating training scheme that includes a novel self-consistency loss for improved text generation based on continuous primers.
%Moreover, the RT architecture naturally scales to multitask regression.



% \subsection{Related work and application domain}
%Due to the success of transformers, abstracting existing problem formulations to sequence modeling is not entirely novel, e.g., the Decision Transformer~\citep{chen2021decision} casts reinforcement learning (RL) as conditional sequence modeling and thus allows to generate appropriate actions by conditioning on desired rewards.
%In this work, we propose to solve regression tasks with sequence models and find that conditioning on numerical property tokens yields a conditional generative model for text sequences.
%While our experiments focus on chemical language modeling (particularly molecular property prediction and property-driven molecular design), we emphasize the generality of the Regression Transformer.
% \vspace{-1mm}
Models that concurrently excel at regression and conditional sequence generation are
beyond applications in NLP
%besides theoretical considerations, 
of special interest for chemo- and bioinformatics.
% \todo{Mention somewhere the applicability to NLP}
Molecules are often labelled with continuous properties (e.g., drug efficacy or protein solubility) and design tasks are intertwined with biochemical properties.
But despite the rise of deep generative models in molecular~\cite{elton2019deep, chen2021deep} and protein design~\cite{wu2021protein,madani2020progen}, current approaches still develop property predictors and generative models independently.
%from another.
%We call this the \textit{explanatory gap of molecular generative models}.
Transformer-based architectures have been used widely on chemical tasks but either focused on property prediction~\citep{wang2019smiles,kim2021merged} or on conditional molecular design~\citep{irwin2021chemformer,mahmood2021masked}, never on both.
This semantic gap persists across architectural flavors (e.g.,~GANs~\citep{mendez2020novo}, RL~\citep{born2021datadriven}, VAEs~\citep{gomez2018automatic}, GNNs~\citep{maziarz2022learning,mahmood2021masked}, flow~\citep{shi2020graphaf} and diffusion models~\citep{jain2022biological}) 
%because the generative sub-modules are always separate from the predictive modules.
To our knowledge, all existing approaches limit the communication between both modules to a reward/loss and thus fail to "entangle" constrained structure generation with property prediction.
By sharing weights between both tasks, the RT adheres to the intuitive expectation that a property-driven generative model should, in the first place, excel at recognizing this property.
%The RT aims to close this gap. 
%while easing the interpretation of property prediction and sample generation by analyzing its attention weights.

\todo{
 - yield: is a generalization of forward reaction and retrosynthesis models 
 - accelerated discovery
 - foundation models
 - SELFIES, devised for generative tasks, have similar predictive power like SMILES
}

% \subsection{Experimental scope} 
% From here it is more chemistry related
In the remainder of this paper, we describe the capabilities of the RT 
%which is build upon the XLNet backbone~\citep{yang2019xlnet}.
%The RT is evaluated in 
on a diverse set of predictive and generative tasks in chemical and protein language modeling.
For chemical languages, we first validate the RT on a synthetic dataset of drug-likeness~\citep{bickerton2012quantifying}, and then test it on three property prediction datasets from the MoleculeNet benchmark~\citep{wu2018moleculenet}.
\todo{
The dichotomy of our model makes it challenging to have a good comparison??
}


one property-driven molecular generation benchmark~\citep{jin2018junction}.
For protein sequence modeling, we apply the RT on a synthetic dataset of protein solubility~\citep{boman2003antibacterial} and two regression datasets from TAPE~\citep{rao2019evaluating}.
\todo{Describe how we measure performance on a variety of sequence generation tasks
- adapting molecules or proteins according to a property of interest
- generating novel chemical reactions by replacing a single precursor to obtain a higher yield than the seed reaction
- generating jokes with high similarity to the actual jokes
}

Although we aim to concurrently excel at predicting properties and generating sequences conditioned on properties, we start training with the PLM objective~\citep{yang2019xlnet} which does not explicitly model those tasks.
We then refine this objective and devise a training scheme that alternates between optimizing property prediction and text generation.
For the latter, we derive a novel self-consistency loss that exploits the dichotomy of the RT by querying itself with the generated candidate sequence.
%, similar to a Siamese network.
We compare our results on property prediction with previous approaches relying on a regression loss. %ChemBERTa~\citep{chithrananda2020chemberta},SMILES-BERT~\citep{wang2019smiles} and CHEM-BERT~\citep{kim2021merged}.
%
To assess the conditional sequence generation, we systematically vary the continuous properties and investigate the model's ability to generate sequences that adhere to the primed property.
We show applications on property-driven local chemical space exploration by decorating scaffolds with a continuum of properties and evaluate the novel molecules using the RT itself as well as an independent property predictor~\citep{rong2020self}.

